EffiCoder: Enhancing Code Generation in Large Language Models through Efficiency-Aware Fine-tuning

As large language models (LLMs) play an increasingly important role in code generation, enhancing both correctness and efficiency has become crucial. Current methods primarily focus on correctness, often overlooking efficiency. To address this gap, we introduce EffiCoder to improve both aspects by fine-tuning LLMs on a high-quality dataset comprising correct and efficient code samples. Our methodology involves leveraging multiple LLMs to generate diverse candidate code solutions for various tasks across different programming languages. We then evaluate these solutions by measuring their execution time and memory usage through local execution. The code solution with the lowest execution time and memory consumption is selected as the final output for each task. Experimental results demonstrate significant improvements when fine-tuning with Effi-Instruct. For instance, Qwen2.5-Coder-7B-Instruct's pass@1 score increases from 44.8\% to 57.7\%, while the average execution time for correct tasks decreases by 48.4\%. EffiCoder offers a scalable and effective solution for advancing AI-driven code generation, benefiting software development and computational problem-solving. The source code of Effi-Code was released at https://github.com/huangd1999/EffiCoder.

==> tables/dpo.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Code efficiency and pass@1 of DeepSeek-Coder-6.7B-instruct fine-tuned using ORPO and DPO with the \dataset.}
    \label{tab:dpo}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Overlap (\%) $\uparrow$}&\textbf{Pass@1 (\%) $\uparrow$}\\
\midrule
HumanEval\\
\midrule
% deepseek-coder-6.7b-base&0.39&2.11&60.50&1.00&12.82&2.04&0.6&7.3\\
% ORPO&0.19 ({\color{problemcolor}51.3\%})&1.04 ({\color{problemcolor}50.7\%})&60.70 ({\color{problemcolor}-0.3\%})&1.00 ({\color{problemcolor}0.0\%})&6.60 ({\color{problemcolor}48.5\%})&1.05 ({\color{problemcolor}48.5\%})&0.6&54.9\\
% DPO&0.19 ({\color{problemcolor}51.3\%})&1.04 ({\color{problemcolor}50.7\%})&60.43 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&6.67 ({\color{problemcolor}48.0\%})&1.06 ({\color{problemcolor}48.0\%})&0.6&3.0\\
deepseek-coder-6.7b-instruct&0.64&1.99&63.85&0.98&26.98&1.88&29.3&43.3\\
ORPO&0.43 ({\color{problemcolor}32.8\%})&0.99 ({\color{problemcolor}50.3\%})&63.74 ({\color{problemcolor}0.2\%})&0.98 ({\color{problemcolor}0.0\%})&20.64 ({\color{problemcolor}23.5\%})&1.00 ({\color{problemcolor}46.8\%})&29.3&71.3\\
DPO&0.44 ({\color{problemcolor}31.2\%})&1.00 ({\color{problemcolor}49.7\%})&63.78 ({\color{problemcolor}0.1\%})&0.98 ({\color{problemcolor}0.0\%})&21.11 ({\color{problemcolor}21.8\%})&1.02 ({\color{problemcolor}45.7\%})&29.3&55.5\\
% Qwen2.5-Coder-7B&0.42&2.04&62.83&1.00&13.63&1.87&14.6&63.4\\
% ORPO&0.20 ({\color{problemcolor}52.4\%})&0.99 ({\color{problemcolor}51.5\%})&62.83 ({\color{problemcolor}0.0\%})&1.00 ({\color{problemcolor}0.0\%})&7.16 ({\color{problemcolor}47.5\%})&0.99 ({\color{problemcolor}47.1\%})&14.6&59.8\\
% DPO&0.21 ({\color{problemcolor}50.0\%})&1.02 ({\color{problemcolor}50.0\%})&62.71 ({\color{problemcolor}0.2\%})&1.00 ({\color{problemcolor}0.0\%})&7.24 ({\color{problemcolor}46.9\%})&1.00 ({\color{problemcolor}46.5\%})&14.6&27.4\\
% Qwen2.5-Coder-7B-Instruct&0.76&2.72&62.94&1.00&36.41&3.19&48.8&54.3\\
% ORPO&0.54 ({\color{problemcolor}28.9\%})&1.67 ({\color{problemcolor}38.6\%})&62.87 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&29.08 ({\color{problemcolor}20.1\%})&2.17 ({\color{problemcolor}32.0\%})&48.8&81.7\\
% DPO&0.54 ({\color{problemcolor}28.9\%})&1.71 ({\color{problemcolor}37.1\%})&76.51 ({\color{problemcolor}-21.6\%})&1.23 ({\color{problemcolor}-23.0\%})&95.78 ({\color{problemcolor}-163.1\%})&13.24 ({\color{problemcolor}-315.0\%})&48.8&83.5\\

% \midrule
% EffiBench\\
% \midrule
% deepseek-coder-6.7b-base&0.17&1.06&46.89&1.00&13.31&1.05&4.9&8.5\\
% ORPO&0.16 ({\color{problemcolor}5.9\%})&0.99 ({\color{problemcolor}6.6\%})&46.90 ({\color{problemcolor}-0.0\%})&1.00 ({\color{problemcolor}0.0\%})&11.18 ({\color{problemcolor}16.0\%})&1.00 ({\color{problemcolor}4.8\%})&4.9&57.4\\
% DPO&0.16 ({\color{problemcolor}5.9\%})&1.00 ({\color{problemcolor}5.7\%})&46.19 ({\color{problemcolor}1.5\%})&0.99 ({\color{problemcolor}1.0\%})&13.73 ({\color{problemcolor}-3.2\%})&1.01 ({\color{problemcolor}3.8\%})&4.9&17.5\\
% deepseek-coder-6.7b-instruct&0.11&0.98&24.86&1.00&1.82&0.96&0.6&1.3\\
% ORPO&0.11 ({\color{problemcolor}0.0\%})&0.99 ({\color{problemcolor}-1.0\%})&24.87 ({\color{problemcolor}-0.0\%})&1.00 ({\color{problemcolor}0.0\%})&1.84 ({\color{problemcolor}-1.1\%})&0.99 ({\color{problemcolor}-3.1\%})&0.6&45.5\\
% DPO&0.11 ({\color{problemcolor}0.0\%})&0.95 ({\color{problemcolor}3.1\%})&24.88 ({\color{problemcolor}-0.1\%})&1.00 ({\color{problemcolor}0.0\%})&1.79 ({\color{problemcolor}1.6\%})&0.95 ({\color{problemcolor}1.0\%})&0.6&31.6\\
% Qwen2.5-Coder-7B&0.16&1.02&45.14&1.00&16.90&1.02&13.1&50.1\\
% ORPO&0.15 ({\color{problemcolor}6.3\%})&0.96 ({\color{problemcolor}5.9\%})&45.11 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&15.86 ({\color{problemcolor}6.2\%})&0.96 ({\color{problemcolor}5.9\%})&13.1&62.9\\
% DPO&0.15 ({\color{problemcolor}6.3\%})&0.97 ({\color{problemcolor}4.9\%})&45.11 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&16.07 ({\color{problemcolor}4.9\%})&0.97 ({\color{problemcolor}4.9\%})&13.1&17.7\\
% Qwen2.5-Coder-7B-Instruct&0.47&4.23&31.18&1.00&11.18&5.86&2.9&3.3\\
% ORPO&0.12 ({\color{problemcolor}74.5\%})&0.99 ({\color{problemcolor}76.6\%})&31.19 ({\color{problemcolor}-0.0\%})&1.00 ({\color{problemcolor}0.0\%})&2.80 ({\color{problemcolor}75.0\%})&0.98 ({\color{problemcolor}83.3\%})&2.9&43.3\\
% DPO&0.47 ({\color{problemcolor}0.0\%})&4.20 ({\color{problemcolor}0.7\%})&31.17 ({\color{problemcolor}0.0\%})&1.00 ({\color{problemcolor}0.0\%})&11.24 ({\color{problemcolor}-0.5\%})&5.79 ({\color{problemcolor}1.2\%})&2.9&59.0\\
\bottomrule
    \end{tabular}}
\end{table*}




==> tables/efficient_and_canonical_solution.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Evaluation results for different teacher models of the \dataset fine-tune dataset.}
    \label{tab:comparison}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Overlap (\%) $\uparrow$}&\textbf{Pass@1 (\%) $\uparrow$}\\
\midrule

DeepSeek-Coder-6.7b-base&0.39&2.00&62.52&1.01&12.78&1.85&1.8&7.3\\
Canonical Solution&0.42 ({\color{problemcolor}-7.7\%})&2.12 ({\color{problemcolor}-6.0\%})&62.16 ({\color{problemcolor}0.6\%})&1.00 ({\color{problemcolor}1.0\%})&14.91 ({\color{problemcolor}-16.7\%})&2.15 ({\color{problemcolor}-16.2\%})&1.8&15.2\\
\dataset&0.23 ({\color{problemcolor}41.0\%})&1.19 ({\color{problemcolor}40.5\%})&62.40 ({\color{problemcolor}0.2\%})&1.00 ({\color{problemcolor}1.0\%})&8.31 ({\color{problemcolor}35.0\%})&1.21 ({\color{problemcolor}34.6\%})&1.8&59.8\\
\midrule
DeepSeek-Coder-6.7b-instruct&0.44&2.07&62.47&1.00&15.95&2.11&31.1&43.3\\
Canonical Solution&0.45 ({\color{problemcolor}-2.3\%})&2.11 ({\color{problemcolor}-1.9\%})&62.48 ({\color{problemcolor}-0.0\%})&1.00 ({\color{problemcolor}0.0\%})&16.92 ({\color{problemcolor}-6.1\%})&2.23 ({\color{problemcolor}-5.7\%})&31.1&57.3\\
\dataset&0.27 ({\color{problemcolor}38.6\%})&1.25 ({\color{problemcolor}39.6\%})&62.48 ({\color{problemcolor}-0.0\%})&1.00 ({\color{problemcolor}0.0\%})&11.81 ({\color{problemcolor}26.0\%})&1.45 ({\color{problemcolor}31.3\%})&31.1&76.8\\
\bottomrule
    \end{tabular}}
\end{table*}




==> tables/model_size.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Efficiency and pass@1 results for different sizes of DeepSeek-Coder models.}
    \label{tab:model_size}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Overlap (\%) $\uparrow$}&\textbf{Pass@1 (\%) $\uparrow$}\\
\midrule	

Qwen2.5-Coder-1.5B&0.40&2.95&35.34&1.03&15.68&3.51&27.1&39.6\\
+ SFT&0.22 (({\color{problemcolor}45.0\%})&1.60 (({\color{problemcolor}45.8\%})&34.58 (({\color{problemcolor}2.2\%})&1.00 (({\color{problemcolor}2.9\%})&9.09 (({\color{problemcolor}42.0\%})&1.98 (({\color{problemcolor}43.6\%})&27.1&41.7\\
Qwen2.5-Coder-3B&0.43&2.73&48.73&1.00&33.88&2.59&16.9&31.2\\
+ SFT&0.23 (({\color{problemcolor}46.5\%})&1.60 (({\color{problemcolor}41.4\%})&49.18 (({\color{problemcolor}-0.9\%})&1.00 (({\color{problemcolor}0.0\%})&18.31 (({\color{problemcolor}46.0\%})&1.98 (({\color{problemcolor}23.6\%})&16.9&34.2\\
Qwen2.5-Coder-7B&0.26&1.81&38.88&1.01&18.63&3.01&41.4&50.1\\
+ SFT&0.17 (({\color{problemcolor}34.6\%})&1.23 (({\color{problemcolor}32.0\%})&38.61 (({\color{problemcolor}0.7\%})&1.00 (({\color{problemcolor}1.0\%})&10.82 (({\color{problemcolor}41.9\%})&1.32 (({\color{problemcolor}56.1\%})&41.4&57.3\\
Qwen2.5-Coder-14B&0.36&2.73&32.41&1.00&12.59&2.57&50.1&57.5\\
+ SFT&0.15 (({\color{problemcolor}58.3\%})&1.14 (({\color{problemcolor}58.2\%})&32.41 (({\color{problemcolor}0.0\%})&1.00 (({\color{problemcolor}0.0\%})&6.80 (({\color{problemcolor}46.0\%})&1.23 (({\color{problemcolor}52.1\%})&50.1&63.6\\
\bottomrule
    \end{tabular}}
\end{table*}



==> tables/other_tasks.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Code Efficiency results when we added filtered tasks in Step 5 and Step 6.}
    \label{tab:other_tasks}
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s)}&\textbf{NET}&\textbf{MU (Mb)}&\textbf{NMU}&\textbf{TMU (Mb*s)}&\textbf{NTMU}&\textbf{Global Pass@1}&\textbf{Pass@1}\\
\midrule
\multicolumn{8}{c}{HumanEval}\\
\midrule
Pre- Step 5\\
Pre- Step 6\\
Post Step 6\\
\midrule
\multicolumn{8}{c}{EffiBench}\\
\midrule
Pre- Step 5\\
Pre- Step 6\\
Post Step 6\\
\bottomrule
    \end{tabular}
\end{table*}




==> tables/size.tex <==
% \begin{table*}\scriptsize
%     \centering
%     \caption{Code efficiency and pass@1 of LLMs with DeepSeek-Coder-6.7B-base (Base) and DeepSeek-Coder-6.7B-instruct (Instruct) fine-tuned by \dataset. The percentage in the brackets indicates the extent of the reduction for each respective item. We evaluate the global pass@1 by directly analyzing tasks addressed by both pre-finetuned LLM and \textbf{individual} fine-tuned LLM with specific ratio.}
%     \label{tab:size_individual}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lrrrrrrrr}
% \toprule
% Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Global $\uparrow$}&\textbf{Pass@1 $\uparrow$}\\
% \midrule
% Base&0.89&2.07&67.50&1.00&56.66&1.96&7.3&7.3\\
% 25&0.70 ({\color{problemcolor}21.3\%})&2.37 ({\color{problemcolor}-14.5\%})&63.23 ({\color{problemcolor}6.3\%})&0.99 ({\color{problemcolor}1.0\%})&33.13 ({\color{problemcolor}41.5\%})&2.47 ({\color{problemcolor}-26.0\%})&55.5&55.5\\
% 50&0.60 ({\color{problemcolor}32.6\%})&2.09 ({\color{problemcolor}-1.0\%})&62.67 ({\color{problemcolor}7.2\%})&0.99 ({\color{problemcolor}1.0\%})&26.66 ({\color{problemcolor}52.9\%})&2.11 ({\color{problemcolor}-7.7\%})&54.3&54.3\\
% 75&0.60 ({\color{problemcolor}32.6\%})&2.12 ({\color{problemcolor}-2.4\%})&63.24 ({\color{problemcolor}6.3\%})&0.99 ({\color{problemcolor}1.0\%})&27.51 ({\color{problemcolor}51.4\%})&2.16 ({\color{problemcolor}-10.2\%})&54.3&54.3\\
% 100&0.33 ({\color{problemcolor}62.9\%})&1.24 ({\color{problemcolor}40.1\%})&63.03 ({\color{problemcolor}6.6\%})&1.00 ({\color{problemcolor}0.0\%})&16.54 ({\color{problemcolor}70.8\%})&1.36 ({\color{problemcolor}30.6\%})&59.8&59.8\\
% \midrule
% Instruct&0.81&2.73&63.24&0.99&37.88&3.31&43.3&43.3\\
% 25&0.66 ({\color{problemcolor}18.5\%})&2.30 ({\color{problemcolor}15.8\%})&63.33 ({\color{problemcolor}-0.1\%})&0.99 ({\color{problemcolor}0.0\%})&30.15 ({\color{problemcolor}20.4\%})&2.28 ({\color{problemcolor}31.1\%})&71.3&71.3\\
% 50&0.74 ({\color{problemcolor}8.6\%})&2.73 ({\color{problemcolor}0.0\%})&62.85 ({\color{problemcolor}0.6\%})&0.99 ({\color{problemcolor}0.0\%})&35.24 ({\color{problemcolor}7.0\%})&3.23 ({\color{problemcolor}2.4\%})&72.0&72.0\\
% 75&0.67 ({\color{problemcolor}17.3\%})&2.34 ({\color{problemcolor}14.3\%})&63.46 ({\color{problemcolor}-0.3\%})&0.99 ({\color{problemcolor}0.0\%})&30.82 ({\color{problemcolor}18.6\%})&2.46 ({\color{problemcolor}25.7\%})&73.8&73.8\\
% 100&0.47 ({\color{problemcolor}42.0\%})&1.45 ({\color{problemcolor}46.9\%})&63.14 ({\color{problemcolor}0.2\%})&0.99 ({\color{problemcolor}0.0\%})&25.13 ({\color{problemcolor}33.7\%})&1.77 ({\color{problemcolor}46.5\%})&76.8&76.8\\
% \bottomrule
%     \end{tabular}}
% \end{table*}




% \begin{table*}\scriptsize
%     \centering
%     \caption{Efficiency and pass@1 results for DeepSeek-Coder-6.7B-base/instruct fine-tuned on 25\%, 50\%, 75\%, and 100\% proportions of the \dataset.}
%     \label{tab:size_global}
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lrrrrrrrr}
% \toprule
% Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Overlap (\%) $\uparrow$}&\textbf{Pass@1 (\%) $\uparrow$}\\
% \midrule
% Base&0.99&2.11&69.10&1.00&65.56&1.99&6.1&7.3\\
% 25&0.97 ({\color{problemcolor}2.0\%})&1.96 ({\color{problemcolor}7.1\%})&69.02 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&66.00 ({\color{problemcolor}-0.7\%})&1.97 ({\color{problemcolor}1.0\%})&6.1&55.5\\
% 50&0.98 ({\color{problemcolor}1.0\%})&2.03 ({\color{problemcolor}3.8\%})&68.78 ({\color{problemcolor}0.5\%})&1.00 ({\color{problemcolor}0.0\%})&65.03 ({\color{problemcolor}0.8\%})&1.90 ({\color{problemcolor}4.5\%})&6.1&54.3\\
% 75&0.95 ({\color{problemcolor}4.0\%})&1.93 ({\color{problemcolor}8.5\%})&68.85 ({\color{problemcolor}0.4\%})&1.00 ({\color{problemcolor}0.0\%})&64.17 ({\color{problemcolor}2.1\%})&1.89 ({\color{problemcolor}5.0\%})&6.1&54.3\\
% 100&0.80 ({\color{problemcolor}19.2\%})&1.13 ({\color{problemcolor}46.4\%})&69.01 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&62.14 ({\color{problemcolor}5.2\%})&1.15 ({\color{problemcolor}42.2\%})&6.1&59.8\\

% \midrule
% Instruct&0.42&1.99&62.52&1.00&14.78&1.89&32.9&43.3\\
% 25&0.43 ({\color{problemcolor}-2.4\%})&2.02 ({\color{problemcolor}-1.5\%})&62.45 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&15.06 ({\color{problemcolor}-1.9\%})&1.91 ({\color{problemcolor}-1.1\%})&32.9&71.3\\
% 50&0.41 ({\color{problemcolor}2.4\%})&1.94 ({\color{problemcolor}2.5\%})&62.44 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&14.41 ({\color{problemcolor}2.5\%})&1.84 ({\color{problemcolor}2.6\%})&32.9&72.0\\
% 75&0.42 ({\color{problemcolor}0.0\%})&1.96 ({\color{problemcolor}1.5\%})&62.45 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}0.0\%})&14.61 ({\color{problemcolor}1.2\%})&1.85 ({\color{problemcolor}2.1\%})&32.9&73.8\\
% 100&0.24 ({\color{problemcolor}42.9\%})&1.09 ({\color{problemcolor}45.2\%})&62.56 ({\color{problemcolor}-0.1\%})&1.00 ({\color{problemcolor}0.0\%})&10.10 ({\color{problemcolor}31.7\%})&1.15 ({\color{problemcolor}39.2\%})&32.9&76.8\\
% \bottomrule
%     \end{tabular}}
% \end{table*}




==> tables/source.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Code efficiency and pass@1 of LLMs with \name . The percentage in the brackets indicates the extent of the reduction for each respective item. Top performing LLMs are highlighted.}
    \label{tab:source}
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Global $\uparrow$}&\textbf{Pass@1 $\uparrow$}\\
\midrule
\multicolumn{8}{c}{HumanEval}\\
\midrule
Base&0.22&1.05&62.97&1.00&7.94&1.10&3.0&3.0\\
Apps&0.23&1.10&68.69&1.00&8.54&1.05&1.2&27.4\\
Dolphin&0.20&1.01&63.01&1.00&7.09&0.99&1.8&22.6\\
Glaive&0.19&0.80&59.18&1.00&6.23&0.89&0.6&4.9\\
Evol-Ins&0.20&0.95&63.94&1.00&7.01&0.96&2.4&39.0\\
Oss-Ins&0.20&0.99&59.39&1.00&6.60&1.00&1.8&1.8\\
Self-Oss&0.21&1.03&67.48&1.00&7.87&1.03&0.6&22.0\\
Alpaca&0.19&0.79&59.45&1.01&6.22&0.89&0.6&4.3\\
CodeFeedback&0.20&1.01&65.03&1.00&7.18&0.99&1.2&40.2\\
Evol-Ins + CodeFeedback&0.22&0.99&64.49&1.00&7.77&1.00&1.2&52.4\\
\bottomrule
    \end{tabular}
\end{table*}




==> tables/teacher.tex <==
\begin{table*}\scriptsize
    \centering
    \caption{Comparison of code efficiency and pass@1 between different teacher models.}
    \label{tab:teacher}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lrrrrrrrr}
\toprule
Model&\textbf{ET (s) $\downarrow$} &\textbf{NET $\downarrow$}&\textbf{MU (Mb) $\downarrow$}&\textbf{NMU $\downarrow$}&\textbf{TMU (Mb*s) $\downarrow$}&\textbf{NTMU $\downarrow$}&\textbf{Overlap (\%) $\uparrow$}&\textbf{Pass@1 (\%) $\uparrow$}\\
\midrule

DeepSeek-Coder-6.7B-base&1.38&2.16&72.86&1.00&99.37&1.95&3.7&7.3\\

Claude-3.5-Sonnet&1.11 ({\color{problemcolor}19.6\%})&1.02 ({\color{problemcolor}52.8\%})&72.83 ({\color{problemcolor}0.0\%})&1.00 ({\color{problemcolor}0.0\%})&92.07 ({\color{problemcolor}7.3\%})&1.03 ({\color{problemcolor}47.2\%})&3.7&29.9\\

GPT-4o&1.10 ({\color{problemcolor}20.3\%})&0.99 ({\color{problemcolor}54.2\%})&72.63 ({\color{problemcolor}0.3\%})&1.00 ({\color{problemcolor}0.0\%})&91.76 ({\color{problemcolor}7.7\%})&0.99 ({\color{problemcolor}49.2\%})&3.7&39.0\\

DeepSeek-Coder-V2-Lite (Ours)&1.16 ({\color{problemcolor}15.9\%})&1.06 ({\color{problemcolor}50.9\%})&72.90 ({\color{problemcolor}-0.1\%})&1.00 ({\color{problemcolor}0.0\%})&97.47 ({\color{problemcolor}1.9\%})&1.08 ({\color{problemcolor}44.6\%})&3.7&59.8\\

\midrule

Instruct&0.41&2.01&65.38&1.01&14.37&1.93&0.6&43.3\\

Claude-3.5-Sonnet&0.26 ({\color{problemcolor}36.6\%})&1.27 ({\color{problemcolor}36.8\%})&65.24 ({\color{problemcolor}0.2\%})&1.00 ({\color{problemcolor}1.0\%})&9.45 ({\color{problemcolor}34.2\%})&1.27 ({\color{problemcolor}34.2\%})&0.6&11.0\\


GPT-4o&0.20 ({\color{problemcolor}51.2\%})&0.98 ({\color{problemcolor}51.2\%})&65.13 ({\color{problemcolor}0.4\%})&1.00 ({\color{problemcolor}1.0\%})&7.34 ({\color{problemcolor}48.9\%})&0.98 ({\color{problemcolor}49.2\%})&0.6&9.8\\

DeepSeek-Coder-V2-Lite (Ours)&0.21 ({\color{problemcolor}48.8\%})&1.04 ({\color{problemcolor}48.3\%})&65.31 ({\color{problemcolor}0.1\%})&1.00 ({\color{problemcolor}1.0\%})&7.76 ({\color{problemcolor}46.0\%})&1.04 ({\color{problemcolor}46.1\%})&0.6&76.8\\
\bottomrule
    \end{tabular}}
\end{table*}
